Data-Efficient Collaborative Decentralized Thermal-Inertial Odometry

We propose a system solution to achieve data-efficient, decentralized state estimation for a team of flying robots using thermal images and inertial measurements. Each robot can fly independently, and exchange data when possible to refine its state estimate. Our system front-end applies an online photometric calibration to refine the thermal images so as to enhance feature tracking and place recognition. Our system back-end uses a covariance-intersection fusion strategy to neglect the cross-correlation between agents so as to lower memory usage and computational cost. The communication pipeline uses Vector of Locally Aggregated Descriptors (VLAD) to construct a request-response policy that requires low bandwidth usage. We test our collaborative method on both synthetic and real-world data. Our results show that the proposed method improves by up to 46 % trajectory estimation with respect to an individual-agent approach, while reducing up to 89 % the communication exchange. Datasets and code are released to the public, extending the already-public JPL xVIO library.

==> sections/macros.tex <==
\global\long\def\bu{\mathbf{u}}
\global\long\def\bx{\mathbf{x}}
\global\long\def\bp{\mathbf{p}}
\global\long\def\bparams{\mathbf{p}}
\global\long\def\Rot{\mathtt{R}}
\global\long\def\bt{\mathbf{t}}
\global\long\def\pol{p}
\global\long\def\velflow{\mathbf{v}}
\global\long\def\linvel{\mathbf{V}}
\global\long\def\angvel{\boldsymbol{\omega}}

\global\long\def\Real{\mathbb{R}}
\global\long\def\cF{\mathcal{F}}

\global\long\def\Patch{\Omega}

\RequirePackage{isomath}
\renewcommand{\vec}{\vectorsym}
\newcommand{\mat}{\matrixsym}

\usepackage{mathtools}
\DeclarePairedDelimiter\norm{\lVert}{\rVert}
\newcommand{\pre}[2]{\prescript{}{#1}{#2}}

\newcommand{\map}[0]{\mathcal{M}}
\newcommand{\domain}[0]{\mathcal{U}}
\newcommand{\deltapose}[0]{\delta\vec{T}}
\newcommand{\pose}[0]{\vec{T}}
\newcommand{\vel}[0]{\dot{\pose}}
\newcommand{\px}[0]{\vec{u}}
\newcommand{\predI}[1]{\hat{I}(#1)}
\newcommand{\predDelta}[1]{\Delta\predI{#1}}
\newcommand{\obsDelta}[1]{\Delta{}I(#1)}
\newcommand{\events}[0]{\{e_k\}}

\global\long\def\regParam{\pose}

\newcommand{\state}{\boldsymbol{x}}
\newcommand{\deltastate}{\delta\boldsymbol{x}}
\newcommand{\sxi}{\boldsymbol{x}_I}
\newcommand{\deltaxi}{\delta\boldsymbol{x}_I}
\newcommand{\xv}{\boldsymbol{x}_V}
\newcommand{\deltaxv}{\delta\boldsymbol{x}_V}
\newcommand{\xs}{\boldsymbol{x}_S}
\newcommand{\deltaxs}{\delta\boldsymbol{x}_S}
\newcommand{\xf}{\boldsymbol{x}_F}
\newcommand{\deltaxf}{\delta\boldsymbol{x}_F}

\newcommand{\pos}[2]{\boldsymbol{p}_{#1}^{#2}}
\newcommand{\quat}[2]{\boldsymbol{q}_{#1}^{#2}}
\newcommand{\tangle}[2]{\boldsymbol{\theta}_{#1}^{#2}}
\newcommand{\estpos}[2]{\boldsymbol{\hat{p}}_{#1}^{#2}}
\newcommand{\estquat}[2]{\boldsymbol{\hat{q}}_{#1}^{#2}}
\newcommand{\esttangle}[2]{\boldsymbol{\hat{\theta}}_{#1}^{#2}}

\newcommand{\deltaresidualbar}{\delta\bar{\boldsymbol{z}}}
\newcommand{\deltaresidual}{\delta\boldsymbol{z}}
\newcommand{\residual}{\boldsymbol{z}}
\newcommand{\residualp}[3]{{}^{#1}\residual_{#2}^{#3}}
\newcommand{\deltaresidualp}[3]{{}^{#1}\deltaresidual_{#2}^{#3}}
\newcommand{\deltaresidualbarp}[3]{{}^{#1}\deltaresidualbar_{#2}^{#3}}

\newcommand{\deltawpf}{{}^w{\delta\boldsymbol{p}_j}}
\newcommand{\wpf}{{}^w{\boldsymbol{p}_j}}
\newcommand{\wpfp}[1]{{}^w{\boldsymbol{p}_j}^{#1}}

\newcommand{\pawp}[1]{{}^w{\boldsymbol{p}_{a_j}^{#1}}}
\newcommand{\qawp}[1]{{}^w{\boldsymbol{p}_{a_j}^{#1}}}
\newcommand{\Cawp}[1]{\boldsymbol{C}(\qawp{#1})}



\newcommand{\jacob}[3]{{}^{#1}\boldsymbol{H}_{#2}^{#3}}
\newcommand{\jacobbar}[3]{{}^{#1}\bar{\boldsymbol{H}}_{#2}^{#3}}

\newcommand{\figref}[1]{Figure~\ref{#1}}


\newcommand{\changes}[1]{{#1}} %

